On the Effective Horizon of Inverse Reinforcement Learning

Inverse reinforcement learning (IRL) algorithms often rely on (forward) reinforcement learning or planning, over a given time horizon, to compute an approximately optimal policy for a hypothesized reward function; they then match this policy with expert demonstrations. The time horizon plays a critical role in determining both the accuracy of reward estimates and the computational efficiency of IRL algorithms. Interestingly, an *effective time horizon* shorter than the ground-truth value often produces better results faster. This work formally analyzes this phenomenon and provides an explanation: the time horizon controls the complexity of an induced policy class and mitigates overfitting with limited data. This analysis provides a guide for the principled choice of the effective horizon for IRL. It also prompts us to re-examine the classic IRL formulation: it is more natural to learn jointly the reward and the effective horizon rather than the reward alone with a given horizon. To validate our findings, we implement a cross-validation extension and the experimental results support the theoretical analysis. The project page and code are publicly available.

==> tables/ablate_gt_gamma.tex <==
\begin{table}
    \centering
    \caption{Performance of LP-IRL under different ground-truth discount factors $\gtGamma \in [0.1, 0.3, 0.5, 0.7, 0.9]$ across four Objectworld-X-Objects environments with $X = 25, 50, 75, 100$. We use the number of the objects $X$ to control the complexity of the policy. Intuitively, the larger the number $X$ of the objects, the denser the rewards are, therefore there are more potentially optimal policies. 
     For each task, we present the ground-truth reward function on the left. On the right, we illustrate the ground-truth value functions (row 1), the expert policies (row 2), the average error count curves for a \textbf{batch} of 5 MDPs (row 2) for varies ground-truth discount factor. The vertical dashed lines depict the ground-truth discount factors. }
    \begin{tabular}{c}\hspace{-5mm}
        \includegraphics[width=1\textwidth]{fig/gt_gamma/env_summary_N_100_batch.jpg}
        \\ \hspace{-5mm}       
          \includegraphics[width=1\textwidth]{fig/gt_gamma/env_summary_N_75_batch.jpg}
            \\ \hspace{-5mm}
        
        \includegraphics[width=1\textwidth]{fig/gt_gamma/env_summary_N_50_batch.jpg}
        \\ \hspace{-5mm}
    
        \includegraphics[width=1\textwidth]{fig/gt_gamma/env_summary_N_25_batch.jpg}
    \end{tabular}
    \label{fig:gt_gammas}
    \Description{Varying Gt discount factors}
\end{table}



==> tables/cross_validate.tex <==
\begin{table*}[h]
    \centering
    \begin{tabular}{c}
\hspace{-5mm}
\includegraphics[width=1.05\textwidth]{fig/lp/gridworld/Gridworld-Simple_cross.jpg}
         \\ \hspace{-5mm}
         
      \includegraphics[width=1.05\textwidth]{fig/lp/gridworld/Gridworld-Hard_cross.jpg}
        \\ \hspace{-5mm}
        
        \includegraphics[width=1.05\textwidth]{fig/lp/objectworld/Objectworld-Linear_cross.jpg}
        \\ \hspace{-5mm}
        
        \includegraphics[width=1.05\textwidth]{fig/lp/objectworld/Objectworld-Non-linear_cross.jpg}
    \end{tabular}
    \caption{Using cross-validation to select $( \optimalR, \optimalGamma )$. The green curves are the ground truth error counts and the blue are for the validation error. The red markers highlight the top 10 best $\learnedGamma$s based on the ground-truth errors, while the orange markers highlights that based on the validation error. We only have access to the validation error curves when selecting $\optimalGamma$. 
    }
    \label{fig:cross_validate}
    \Description{CV}
\end{table*}


